Empirical Evaluation of AI-Assisted Software Package Selection: A Knowledge Graph Approach

Selecting third-party software packages in open-source ecosystems like Python is challenging due to the large number of alternatives and limited transparent evidence for comparison. Generative AI tools are increasingly used in development workflows, but their suggestions often overlook dependency evaluation, emphasize popularity over suitability, and lack reproducibility. This creates risks for projects that require transparency, long-term reliability, maintainability, and informed architectural decisions. This study formulates software package selection as a Multi-Criteria Decision-Making (MCDM) problem and proposes a data-driven framework for technology evaluation. Automated data pipelines continuously collect and integrate software metadata, usage trends, vulnerability information, and developer sentiment from GitHub, PyPI, and Stack Overflow. These data are structured into a decision model representing relationships among packages, domain features, and quality attributes. The framework is implemented in PySelect, a decision support system that uses large language models to interpret user intent and query the model to identify contextually appropriate packages. The approach is evaluated using 798,669 Python scripts from 16,887 GitHub repositories and a user study based on the Technology Acceptance Model. Results show high data extraction precision, improved recommendation quality over generative AI baselines, and positive user evaluations of usefulness and ease of use. This work introduces a scalable, interpretable, and reproducible framework that supports evidence-based software selection using MCDM principles, empirical data, and AI-assisted intent modeling.

==> tml.tex <==



These trends point to the need for recommendation systems that go beyond ranking packages by popularity. Several studies have shown that popularity metrics may favor well-known or well-documented libraries, often overlooking less common but highly relevant alternatives~\cite{mcmillan2012portfolio, zhou2010longterm}. Effective tools must incorporate contextual relevance and domain-specific signals to support more informed discovery. Additionally, the large proportion of non-indexed packages emphasizes the importance of extending recommendation mechanisms beyond curated repositories such as PyPI~\cite{kabir2020pyreco}.

Security information introduces another dimension of complexity in package selection. Prior work has highlighted that widely adopted software components can contain known vulnerabilities~\cite{zimmermann2019small}. Integrating vulnerability records, such as those from the OSV or CVE databases, enables developers to make informed trade-offs between popularity and risk exposure~\cite{abdalkareem2017developers}.

In comparisons between PySelect and generative AI models, we found that large language models often suggest packages based on documentation quality or name recognition rather than actual usage in software projects. This observation aligns with recent findings showing that LLMs may generate plausible but suboptimal recommendations when not grounded in real-world code usage patterns~\cite{ling2023llm4code}.

Finally, the challenge of mapping developer reviews to formal quality models persists. While sentiment analysis achieved an F1 score of 0.961, mapping user comments to structured attributes from ISO/IEC~25010 yielded only moderate alignment (F1 score of 0.728). This gap suggests that while user-generated content holds valuable signals, effective quality modeling may require more sophisticated NLP techniques or human-in-the-loop validation~\cite{martin2021capturing}.
